Multi-camera Torso Pose Estimation using Graph Neural Networks

Estimating the location and orientation of humans is an essential skill for service and assistive robots. To achieve a reliable estimation in a wide area such as an apartment, multiple RGBD cameras are frequently used. Firstly, these setups are relatively expensive. Secondly, they seldom perform an effective data fusion using the multiple camera sources at an early stage of the processing pipeline. Occlusions and partial views make this second point very relevant in these scenarios. The proposal presented in this paper makes use of graph neural networks to merge the information acquired from multiple camera sources, achieving a mean absolute error below 125 mm for the location and 10 degrees for the orientation using low-resolution RGB images. The experiments, conducted in an apartment with three cameras, benchmarked two different graph neural network implementations and a third architecture based on fully connected layers. The software used has been released as open-source in a public repository (https://github.com/vangiel/WheresTheFellow).

==> datasets.tex <==
\subsection{Datasets that can be used}

The most relevant datasets for \textbf{2D} labelled images and videos are:

\begin{itemize}
\item Common Objects in Context (COCO) by Microsoft \cite{COCO2014}: This one include RGB images of different objects that are segmented and captioned in most of the dataset. However, it does not include joints annotation. 
\item \textbf{MPII Human Pose Dataset \cite{andriluka14cvpr}} and MPII Human pose Models \cite{pishchulin16cvpr,insafutdinov16ariv}: Both of them include labelled images of joints of the people depicted in them. However, the first one also include annotations of the action performed by that people and an approximation of the 3D coordinates and orientation of the person. This can be useful to this project since it is the kind of dataset used to train the GNN but with only one camera.
\item Leeds Sports Pose Dataset (LSP) \cite{Johnson10}: This dataset contains a large amount of images of sports. Each image has joints annotation which include three parameters: x and y locations and a binary value indicating the visibility of each joint.
\end{itemize}

The most relevant datasets for \textbf{3D} and multi-camera labelled images and and videos are:

\begin{itemize}
\item SALSA dataset \cite{7313015}: It contains video frames from four different calibrated RGB cameras operating at 15 frames per second. The position, head and body orientation of each target is annotated every 45 frames (3 seconds). It has other annotations for social interaction analyses such as audio  and personal information about the participants.
\item NTU-RGBD and NTU-RGBD-120 datasets \cite{Liu_2019_NTURGBD120, Shahroudy_2016_NTURGBD}: These two datasets both contain RGB videos, depth map sequences, 3D skeletal data, and infrared (IR) videos for each sample. Each dataset is captured by three Kinect V2 cameras concurrently.  The resolutions of RGB videos are 1920x1080, depth maps and IR videos are all in 512x424, and 3D skeletal data contains the 3D coordinates of 25 body joints at each frame.
\item Human 3.6 \cite{h36m_pami}: 

\end{itemize}

